Planning with Probabilistic Opacity and Transparency: A Computational Model of Opaque/Transparent Observations

Qualitative opacity of a secret is a security property, which means that a system trajectory satisfying the secret is observation-equivalent to a trajectory violating the secret. In this paper, we study how to synthesize a control policy that maximizes the probability of a secret being made opaque against an eavesdropping attacker/observer, while subject to other task performance constraints. In contrast to existing belief-based approach for opacity-enforcement, we develop an approach that uses the observation function, the secret, and the model of the dynamical systems to construct a so-called opaque-observations automaton which accepts the exact set of observations that enforce opacity. Leveraging this opaque-observations automaton, we can reduce the optimal planning in Markov decision processes(MDPs) for maximizing probabilistic opacity or its dual notion, transparency, subject to task constraints into a constrained planning problem over an augmented-state MDP. Finally, we illustrate the effectiveness of the developed methods in robot motion planning problems with opacity or transparency requirements.

==> power_plant_example_task_spec_dfa.tex <==
% \documentclass[varwidth]{standalone}

% \usepackage{graphicx}
% \usepackage{changes}
% \usepackage[utf8]{inputenc}
% \usepackage{comment}
% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{amssymb}
% \usepackage{acronym}
% \usepackage{xcolor}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usetikzlibrary{shapes,arrows,fit,backgrounds,automata}
% \usetikzlibrary{shapes.geometric,fit}
% \usepackage{mathtools}
% \usepackage{paralist}
% \usepackage{tikz}
% \usetikzlibrary{external}
% \tikzexternalize % activate!

% \begin{document}


\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.5cm,scale=0.7,semithick, transform shape]

    \tikzstyle{every state}=[fill=black!10!white];
    \node[state, initial] (1) at (-3, -0.5) {$p_1$};
    \node[state, accepting] (2) at (-1.5, -0.5) {$p_2$};
      \path 
        (1) edge [loop above]  node{$\neg \mathbf{C}$} (1)
        (1) edge   node {$\mathbf{C}$} (2)
        (2) edge [loop above]   node{$True$} (2)
        ;
\end{tikzpicture}


% \end{document}
